Precise Photon Arrival Time Measurement via Time to Frequency Demultiplexing

We demonstrate a nonlinear-optics approach to precise measurement of photon arrival time, by translating the temporal information of single photons to a wavelength distribution of frequency conversion followed by de-multiplexed detection. It uses a multi-color, pulse-delayed pump laser to drive multiplexed frequency conversion, transducing photons to various frequency channels according to their arrival time. By photon detection in each channel, the measurement resolution and accuracy can reach picosecond level, much lower than the detectors' naive resolution and significantly beating the shot-noise limited direct detection. Distinct to any method relying on repeated, multiple sampling, our approach supports event-ready operations, capable of detecting randomly arriving single photons with no dead window. It is thus particularly suitable for practical applications of ranging, sensing, and communications in the dynamic, photon-starving environment.

==> images/concept/name.tex <==
\usetikzlibrary{shapes.geometric, arrows.meta, decorations.pathreplacing, calc}

\begin{tikzpicture}[
    scale=0.8,
    font=\sffamily\small,
    >=Stealth,
    spectral_axis/.style={->, thick},
    signal_line/.style={thick, blue!60!black},
    pump_line/.style={thick, magenta},
    pm_line/.style={thick, red},
    box/.style={draw, thick, minimum width=3cm, minimum height=1.5cm}
]

% --- Top Left Inputs ---
% Signal spectra
\draw[spectral_axis] (-6,4) -- (-3.5,4) node[right] {$\lambda$};
\draw[spectral_axis] (-6,4) -- (-6,5);
\draw[signal_line, orange] (-5.8,4) .. controls (-5.6,4.8) and (-5.4,4.8) .. (-5.2,4);
\draw[signal_line, green!60!black] (-5.3,4) .. controls (-5.1,4.8) and (-4.9,4.8) .. (-4.7,4);
\draw[signal_line, cyan] (-4.8,4) .. controls (-4.6,4.8) and (-4.4,4.8) .. (-4.2,4);
\node at (-5.9, 4.5) {\dots};
\node at (-3.8, 4.5) {\dots};

% Pump spectrum
\draw[spectral_axis] (-6,2.5) -- (-3.5,2.5) node[right] {$\lambda$};
\draw[spectral_axis] (-6,2.5) -- (-6,3.5);
\draw[pump_line] (-5.2,2.5) .. controls (-4.9,3.3) and (-4.5,3.3) .. (-4.2,2.5);
\draw[<->] (-5.5,2.8) -- (-3.9,2.8);

% Combine signals
\draw[thick, teal] (-3.5, 4.4) .. controls (-2.5,4.4) and (-2.5,3.7) .. (-2, 3.7);
\draw[thick, teal] (-3.5, 3.0) .. controls (-2.5,3.0) and (-2.5,3.7) .. (-2, 3.7);
\draw[thick, teal] (-2, 3.7) -- (-1, 3.7);

% --- MQPG Center Block ---
\node[box, minimum width=4cm, minimum height=2cm] (MQPG) at (1,3.5) {};
\node at (1, 2.2) {\textbf{MQPG}};
\foreach \x in {-0.6, -0.2, 0.4, 0.8, 1.4, 1.8, 2.2} {
    \draw[thick] (\x, 2.5) -- (\x, 4.5);
}

% --- Phase Matching Curves (Top) ---
\draw[spectral_axis] (0,5.2) -- (3,5.2) node[right] {$\lambda$};
\draw[spectral_axis] (0,5.2) -- (0,6.5) node[above, align=left, font=\scriptsize] {phase\\matching};
\foreach \off in {0.5, 1.3, 2.1} {
    \draw[pm_line] (\off,5.2) .. controls (\off+0.2,6.3) and (\off+0.4,6.3) .. (\off+0.6,5.2);
}
\node[red] at (0.2, 5.5) {\dots};
\node[red] at (2.8, 5.5) {\dots};

% --- DEMUX and Output ---
\draw[thick] (3, 3.7) -- (5, 3.7);
\draw[thick] (5, 2.5) -- (6, 1.5) -- (6, 5.5) -- (5, 4.5) -- cycle;
\node at (5.5, 5.8) {DEMUX};

\foreach \y/\c in {4.8/orange, 3.7/green!60!black, 2.6/cyan} {
    \draw[thick] (6, \y) -- (7.5, \y);
    \draw[spectral_axis] (7.8, \y-0.5) -- (9.5, \y-0.5) node[right, scale=0.7] {$\lambda$};
    \draw[thick, \c] (8.3, \y-0.5) .. controls (8.6, \y+0.2) and (8.9, \y+0.2) .. (9.2, \y-0.5);
}
\node at (8.7, 5.6) {\vdots};
\node at (8.7, 1.8) {\vdots};

% --- Lower Detailed Section (Zoom) ---
\draw[dashed, gray] (MQPG.south west) -- (-2, -1);
\draw[dashed, gray] (MQPG.south east) -- (6, -1);

% Time bins (Row 1)
\foreach \i/\t in {0/0, 1/1, 2/2} {
    \begin{scope}[shift={({-1.5 + \i*3.5}, -2)}]
        \draw[spectral_axis] (0,0) -- (2.5,0) node[right] {$\Delta t$};
        \draw[signal_line, orange] (0.2,0) .. controls (0.4,0.8) and (0.6,0.8) .. (0.8,0);
        \draw[signal_line, green!60!black] (0.7,0) .. controls (0.9,0.8) and (1.1,0.8) .. (1.3,0);
        \draw[signal_line, cyan] (1.2,0) .. controls (1.4,0.8) and (1.6,0.8) .. (1.8,0);
        
        \draw[spectral_axis] (0,-1.5) -- (2.5,-1.5) node[right] {$\Delta t$};
        \draw[pump_line] ({0.5 + \i*0.5},-1.5) .. controls ({0.8 + \i*0.5},-0.7) and ({1.2 + \i*0.5},-0.7) .. ({1.5 + \i*0.5},-1.5);
    \end{scope}
}

% Phase matching bins (Row 2)
\foreach \i in {0, 1, 2} {
    \begin{scope}[shift={({-1.5 + \i*3.5}, -5)}]
        \draw[spectral_axis] (0,0) -- (2.5,0) node[right] {$\lambda$};
        \draw[pm_line] (0.2,0) .. controls (0.5,1.5) and (0.8,1.5) .. (1.1,0);
        \draw[pm_line] (1.0,0) .. controls (1.3,1.5) and (1.6,1.5) .. (1.9,0);
        \draw[pm_line] (1.8,0) .. controls (2.1,1.5) and (2.4,1.5) .. (2.7,0);
        
        % Overlays
        \ifnum\i=0 \draw[thick, orange] (0.3,0) .. controls (0.5,0.8) and (0.8,0.8) .. (1.0,0); \fi
        \ifnum\i=1 \draw[thick, green!60!black] (1.1,0) .. controls (1.3,0.8) and (1.6,0.8) .. (1.8,0); \fi
        \ifnum\i=2 \draw[thick, cyan] (1.9,0) .. controls (2.1,0.8) and (2.4,0.8) .. (2.6,0); \fi
    \end{scope}
}
\node[red, align=left, font=\scriptsize] at (-2.2, -4.2) {phase\\matching};

% --- Connective Arrows ---
\draw[->, teal, bend right=20] (-5, 1.8) to (-2.5, -1.5);
\draw[->, teal, bend right=20] (9, 1) to (9, 3);

\end{tikzpicture}


==> images/setup/mQPG.tex <==
\begin{tikzpicture}[font=\small, line cap=round, line join=round]

% Main waveguide (gray rectangle)
\draw[fill=gray!20, draw=gray!70!black] (0,0.19) rectangle (1,-0.19);

% Periodic vertical sections (white bars) within the waveguide
\foreach \x in {0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8} {
  \draw[fill=white, draw=gray!70!black] (\x,0.15) rectangle (\x+0.05,-0.15);
}
% Two colored outputs from the right side of the waveguide
\draw[thick, green!70!black] (1,0.05) -- (1.2,0.05);
\draw[thick, orange!90!black] (1,0.0) -- (1.2,0.0);
\draw[thick, red!90!black] (1,-0.05) -- (1.2,-0.05);


\draw (1.4,0.25) arc[start angle=-270, end angle=-90, radius=0.25cm] -- ++(0,0.5);




\end{tikzpicture}


==> images/setup/spectrograph.tex <==
\usetikzlibrary{circuits.logic.US, positioning}

\begin{tikzpicture}[font=\sffamily\scriptsize, every node/.style={align=center}, circuitikz/bipoles/length=1cm]
  % Two colored outputs from the right side of the waveguide
\draw[thick, green!70!black] (-1.5,0.1) -- (-1.25,0.1);
\draw[thick, orange!90!black] (-1.5,0) -- (-1.25,0);
\draw[thick, red!90!black] (-1.5,-0.1) -- (-1.25,-0.1);

  % Half-circle with flat right side
  \draw (-1,0.25) arc[start angle=-270, end angle=-90, radius=0.25cm] -- ++(0,0.5);
  \node at (-1,0.75) {Coupler};
  \node at (-2.5,0) {\textbf{mQPG} \\ \textbf{WG}};

  \draw[draw=red, line width=2pt] (-1,0) -- (1.2,0);

  % Diagonal outputs (e.g., LEDs)
  \foreach \i in {0,...,5} {
    \draw (1,0.3) -- ++(\i*0.1,-\i*0.125);
    \filldraw (1,0.3) ++(\i*0.1,-\i*0.125) circle (0.05);
  }
 \node[align=center] at (1.2,1) {Diffraction \\ grating};

  % Vertical lines (each with a label)
  \draw (-1,-1) -- (-1,-2);
  \node at (-1.4,-1.5) {$m_1$};

  \draw (1.2,-2) -- (1.2,-3);
  \node at (1.6,-2.5) {$m_2$};

  \draw (-1,-3) -- (-1,-4);
  \node at (-1.4,-3.5) {$m_3$};

  \draw (1.2,-4) -- (1.2,-5);
  \node at (1.6,-4.5) {$m_4$};

  \draw (-1,-5) -- (-1,-6);
  \node at (-1.4,-6.5) {$m_5$};

  \draw (1.2,-6) -- (1.2,-7);
  \node at (1.6,-7.5) {$m_6$};

  \draw (-1,-7) -- (-1,-7.5);
  \node at (-1.4,-7.75) {$m_7$};

  \draw (-1,-8) -- (-1,-8.5);
  \node at (-1.4,-8.75) {$m_8$};

  \draw (-1,-9) -- (-1,-9.5);
  \node at (-1.4,-9.75) {$m_9$};

  % Green path
  \draw[green!70!black, line width=1.5pt] (1.2,0) -- (-1,-1.4) -- (1.2,-2.3) -- (-1,-3.2) -- (1.2,-4.1) -- (-1,-5.25) -- (1.7,-6.1);

  % Orange path
  \draw[draw=orange!90!black, line width=1.5pt] (1.2,0) -- (-1,-1.5) -- (1.2,-2.45) -- (-1,-3.5) -- (1.2,-4.6) -- (-1,-6.25) -- (1.7,-7.1);

  % Blue path
  \draw[draw=red!90!black, line width=1.5pt] (1.2,0) -- (-1,-1.6) -- (1.2,-2.7) -- (-1,-3.8) -- (1.2,-5) -- (-1,-7.25) -- (1.7,-8.1);

  %% Photodetectors
  \draw (1.7,-5.8) arc[start angle=90, end angle=-90, radius=0.25cm] -- ++(0,0.5);
  \node (c1) at (1.8,-6.1) {};
  \node (spd1) [right=0.2cm of c1, draw, rectangle, minimum width=1cm, minimum height=0.5cm] {SPD$_1$};
  \draw (c1.east)--(spd1.west);
  \draw[draw=green!40!black, line width=1.5pt] (0.9,-5.6) -- (0.8,-6.1);  \draw[draw=green!40!black, line width=1.5pt] (1.1,-5.7) -- (1.0,-6.2);
  \node at (1.2,-6.2) {$f_1$};

  \draw (1.7,-6.8) arc[start angle=90, end angle=-90, radius=0.25cm] -- ++(0,0.5);
  \node (c2) at (1.8,-7.1) {};
  \node (spd2) [right=0.2cm of c2, draw, rectangle, minimum width=1cm, minimum height=0.5cm] {SPD$_2$};
  \draw (c2.east)--(spd2.west);
  \draw[draw=orange!40!black, line width=1.5pt] (0.9,-6.6) -- (0.8,-7.1);
  \node at (1,-7) {};
  \draw[draw=orange!40!black, line width=1.5pt] (1.1,-6.7) -- (1.0,-7.2);
  \node at (1.2,-7.2) {$f_2$};
  
  \draw (1.7,-7.8) arc[start angle=90, end angle=-90, radius=0.25cm] -- ++(0,0.5);
  \node (c3) at (1.8,-8.1) {};
  \node (spd3) [right=0.2cm of c3, draw, rectangle, minimum width=1cm, minimum height=0.5cm] {SPD$_3$};
  \draw (c3.east)--(spd3.west);
  \draw[draw=red!40!black, line width=1.5pt] (0.9,-7.6) -- (0.8,-8.1);
  \node at (1,-8) {};
  \draw[draw=red!40!black, line width=1.5pt] (1.1,-7.7) -- (1.0,-8.2);
  \node at (1.2,-8.2) {$f_3$};

  
  \node (pc) at (4.5,-7.1){\includegraphics[width=1.25cm]{images/setup/PC.png}};
  \node at ($(pc.south)+(0,-0.1)$) {PC};

  \draw (spd1.east) -- (pc.west);
  \draw (spd2.east) -- (pc.west);
  \draw (spd3.east) -- (pc.west);
\end{tikzpicture}

